Mould Calculus for Hamiltonian Vector Fields

We present the general framework of \'Ecalle's moulds in the case of linearization of a formal vector field without and within resonances. We enlighten the power of moulds by their universality, and calculability. We modify then \'Ecalle's technique to fit in the seek of a formal normal form of a Hamiltonian vector field in cartesian coordinates. We prove that mould calculus can also produce successive canonical transformations to bring a Hamiltonian vector field into a normal form. We then prove a Kolmogorov theorem on Hamiltonian vector fields near a diophantine torus in action-angle coordinates using moulds techniques.

==> actionangle.tex <==
%%%%%%%%%%%
%%%%%%
%   coordonnées actions-angles
%
%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
 In this section, we use the preceding trimmed form transformations to bring a Hamiltonian vector field into Kolmogorov's normal form. The Kolmogorov's theorem
ensures the persistence of a diophantine torus of a completely integrable Hamiltonian
function under a weak perturbation. We prove this theorem in the case of a perturbation
of a special form, see \emph{infra}.

 We define the algebra $\mathcal{A}_\epsilon$ of functions $f_\epsilon(p,q):\C\times
 \C\to\C$ of the form $f_\epsilon(p,q)=\sum_{s\geq0} \epsilon^s f_s(p,q)$ where the
 $f_s$ are trigonometric polynomials in $q$, the coefficients  $f_{s,k}(p)$ of which
 being polynomials in $p$, writing $f_s(p,q)= \sum_{|k|\leq K_s}f_{s,k}(p)\expe{k\cdot q}$.
 
  We define $\mathcal{A}^1_\epsilon$ the subset of $\mathcal{A}_\epsilon$ of
  trigonometric polynomials in $q$, the coefficients of which being homogeneous
   polynomials in $p$ of degree $1$.
  
 We denote by $\der(\mathcal{A}_\epsilon)$ the set of derivations over the algebra 
$\mathcal{A}_\epsilon$, and by $\der^1(\mathcal{A}_\epsilon)$ the subset of
$\der(\mathcal{A}_\epsilon)$, of derivations $D$ of the form:
 \eq{ D= A_\epsilon(p,q)\dep_p+B_\epsilon(p,q)\dep_q,}
 with $A_\epsilon(p,q), B_\epsilon(p,q)$ in $\mathcal{A}^1_\epsilon$.
 
 Moreover, we denote by $ \der^1_r(\mathcal{A}_\epsilon)\subset 
 \der^1(\mathcal{A}_\epsilon)$ the subset of derivations
  of the form $ A_\epsilon(p,q)\dep_p + B_\epsilon(p,q)\dep_q$, $A_\epsilon$
  and $B_\epsilon$ being in $\mathcal{A}^1_\epsilon$,  of which all the coefficients of $\epsilon^s, s\leq r$ have no dependence in $q$.

  
  Following~\cite{giorgilli} we deal here with Hamiltonian functions from
   $\R^\nu\times\T^\nu$ to $\R$, where $\T$ is the usual torus $\R/\Z$,
   and $\freq$ a vector of $\R^\nu$ being non-resonant, of the form:
 \eqn{\label{eq:hamiltonien} H_\epsilon(p,q) = \freq\cdot p + \frac{1}{2}p^2 + \epsilon f(q).}
 %
%
 The "formal" Kolmogorov theorem is then:
 \begin{theo}\label{theo:kolmo:hamilton}
 Let $H_\epsilon(p,q)$ be defined as in~\eqref{eq:hamiltonien} and
  $\freq\in\R^\nu$ being diophantine. There exists a canonical
 formal transformation $q=q^\prime + \epsilon\cdots, p=p^\prime + \epsilon\cdots$,
 which brings $H_\epsilon$ into Kolmogorov normal form:
 \eq{ H_\epsilon(p,q)=\freq\cdot p + R(p,q,\epsilon),}
 with $R(p,q,\epsilon)=O(p^2)$.
 \end{theo}
 %
%
More precisely, we will prove the following theorem, denoting by 
 $X_{\epsilon}$ the Hamiltonian vector field coming from
 $H_\epsilon$, and by $X_c$ the constant vector field $\freq\cdot\dep_q$:
\begin{theo}\label{theo:kolmo:champ}
Let us suppose that $X_{\epsilon}$ has been brought into the following form:
 \eq{X_{r,\epsilon}(p,q) = \freq\cdot\dep_q + \sum_{s=1}^r \epsilon^s(a_s(p)\dep_p
      + b_s(p)\dep_q) + \sum_{s\geq r+1} \epsilon^s \biggl( \sum_{l=1}^{N_s}
         a_{s,l}(p)\expe{l\cdot q}\dep_p + \sum_{l=1}^{M_s} b_{s,l}(p) \expe{l\cdot q}
         \dep_q \biggr),}
   where $a_s(p), b_s(p), a_{s,l}(p), b_{s,l}(p)$ are in $\mathcal{A}_\epsilon^1$.
   Then, there exists a canonical transformation
 $q=q^\prime + \epsilon\cdots, p=p^\prime + \epsilon\cdots$,
 such that $X_{r,\epsilon}(p,q)=X_{r+1,\epsilon}(p^\prime,q^\prime)$.
\end{theo}
%
%
The theorem we want to prove  may be rewritten as follows:
\begin{theo}\label{theo:iteration-derivee}
If $X-X_c\in \der^1_r(\mathcal{A}_\epsilon)$, then $\Xsam-X_c \in \der^1_{r+1}(\mathcal{A}_\epsilon)$.
\end{theo}
%
\begin{proof}
We write 
\eq{ X = X_c + \sum_{s=1}^r \epsilon^r X_s^0(p) + \sum_{s\geq r+1} \epsilon^s 
     \biggl( X_s^0(p) + \sum_{k\in\Z^v} X_s^k(p,q) \biggr),}
     where $X_s^0(p)$ is independent of $q$ and $X_s^k(p,q)= \expe{(k\cdot q)}
     \biggl( a_{s,k}(p)\dep_p + b_{s,k}(p)\dep_q \biggr)$.
      
 We set then $B_k = \sum_{s\geq r+1} \epsilon^s X^k_s$ for $k\neq0$ and
 $B_0 = \sum_{s\geq1}\epsilon^s X_s^0$.
%
\begin{lemm}
For $k\in\Z^\nu$, $B_k$ is a homogeneous differential operator of degree $k$ in the 
angles $q$.  Moreover, 
\eq{ X_c B_k = \i (k\cdot\freq) B_k.}
\end{lemm}
%
  We can then write $X = X_c + \sum_{\mot{k}\in A^*}I^{\mot{k}} B_{\mot{k}}$,
  where $A=\Z^\nu$ is the alphabet, and $\moule{I}$ the mould already defined.
  We look for $\Theta=\sum_\bullet\moule{\Theta}\comoule{B}$, with
  $\Theta=\exp(V)$ and $V=\sum_\bullet\moule{V}\comoule{B}$.
  
  The Campbell-Baker-Hausdorff formula ensures that:
 \eqn{\label{eq:cbh}
 \Theta X \inv{\Theta} = X - [X,V] + \dotsm = X_c + \sum_{k\in\Z^\nu} B_k 
 - [X_c,V] + \hot,}
 where $\hot$ stands for higher order (in $\epsilon$) terms.
   Moreover, we set:
   \eq{ \moule{V} = \begin{cases}
                           \frac{1}{\i(k\cdot\freq)} \text{ if $\longueur{\bullet}=1$ and $k\cdot\freq
                           \neq0$;}\\
                           0 \text{ otherwise.}
                           \end{cases}}

  Then, \eq{ [X_c,V] = \sum_{k\in\Z^\nu} V^k [X_c,B_k] 
                             + \sum_{\substack{\mot{k}\in A^*\\ \longueur{\mot{k}}\geq2}}
                                     V^{\mot{k}} [X_c,B_{\mot{k}}] + \dotsm, }
    hence, \eqref{eq:cbh} rewrites:
  \eq{ X_c + 
      \underbrace{\sum_{k\in A} B_k - \sum_{k\in A}\i(\freq k )V^k B_k}_
      {(*)}
       + 
       \underbrace{\sum_{\substack{\mot{k}\in A^*\\ \longueur{\mot{k}}\geq2}} V^{\mot{k}}
         [X_c,B_{\mot{k}}] + \dotsm}_{(**)}}

The term $(**)$ is of order in $\epsilon$ at least $r+2$, therefore we do not worry
about it. The term $(*)$ rewrites:
%
\eq{\sum_{k\in A} \sum_{s\geq r+1} \epsilon^s X^k_s -
      \sum_{k\in A} \i(\freq\cdot k) V^k \biggl( \sum_{s\geq r+1} \epsilon^s X^k_s \biggr),}
%
so, if we choose $V^k= \frac{1}{\i(k\cdot\freq)}$, for $k\cdot\freq\neq0$, this latter
expression vanishes, because $X^k_{r+1}=0$ when $k\cdot\freq=0$ (as $\freq$ is non-resonant).
      

%
%\eq{ [X,X_c] = [X_c,X_c] + \sum_{s=1}^{r-1} \epsilon^s[X_s,X_c] + \sum_{s\geq r}
% \epsilon^s [X_s,X_c].}
%%
%If $X_s(p,q)=A_s(p)\dep_p + B_s(p)\dep_q$ (that is, for $s\leq r-1$), then $[X_s,X_c]=0$.
%Hence
% \eq{ [X,X_c] = \sum_{s\geq r} \epsilon^s [X_s,X_c].}
% 
% 
\end{proof}
%
 We have again our transformation $\simp$ which brings $X$ into $\Xsam$.
 After the projection lemma~\ref{lem:projection} we can write:
 \eq{ \Xsam = X_c + \sum_{r\geq1} \frac{1}{r} \sum_{\mot{k}\in A^*} \Sam^{\mot{k}} 
        B_{[\mot{k}]}.}
 Now we use the following lemma:
%
\begin{lemm}
\eq{ \forall D, \widetilde{D} \in \der^1(\mathcal{A}_\epsilon),\qquad
 [D,\widetilde{D}] \in \der^1(\mathcal{A}_\epsilon).}
\end{lemm}
%
%
That lemma and the projection lemma prove that $\Xsam$ is now  in
 $\der^1_{r+1}(\mathcal{A}_\epsilon)$, hence, by applying iteratively
 theorem~\ref{theo:iteration-derivee}, we are able to prove theorem~\ref{theo:kolmo:champ} therefore theorem~\ref{theo:kolmo:hamilton}.
 
%We write then the Hamiltonian vector field:
% \eq{ X_H = \freq\cdot\dep_q + \sum_{k\in\Z^\nu} \expe{(k\cdot q)} \sum_{s\geq1}
%        \epsilon^s X_k^{(s)}(p),}
%     with $X_k^{(s)}$ polynomial of degree $1$ in $p$.
%     
% We want to make successive transformations to bring this initial Hamiltonian vector
% field into $ \Xnor = \freq\cdot\dep_q + R(p,q,\epsilon),$  where $R(p,q,\epsilon)
% =O(p)$ contains only resonant terms.
%   
%  First, remark there is no linear part, but a \emph{constant} part: $X_c=\freq\cdot\dep_q$.
%  Second, remark that the $X_k^{(s)}$ are Hamiltonian vector fields.
% Now, the problem is to write a good decomposition for the non-constant part of $X_H$.
% We define then the following operators:
% \eq{ B_k = \expe{(k\cdot q)} \sum_{s\geq1} \epsilon^s X_k^{(s)} \text{ for $k\in\Z^\nu.$}}
%%
% Remark that they still are Hamiltonian operators.
%%
%%
%As before, we look for a change of variables given by a substitution operator $\Theta$ of the form $\Theta=\exp(V)$ where $V$ is also a vector field, and we write it:
%\eq{ V = \sum_{s\geq1} \epsilon^s \sum_{k\in\Z^\nu} \expe{(k\cdot q)} V_k^{(s)}(p).}
% We want again a simplification to kill non-resonant terms in $X_H$.
%%
%\begin{prop}
%The alphabet is $\Z^\nu$. Moreover, we define the mould $\moule{V}$ as follows:
%\eq{ \moule{V} = \begin{cases}
%                           \frac{1}{\i(k\cdot\freq)} \text{ if $\longueur{\bullet}=1$ and $k\cdot\freq
%                           \neq0$;}\\
%                           0 \text{ otherwise.}
%                           \end{cases}}
%  The simplification given then by $\Theta X\inv{\Theta}$ where $\Theta=\exp(V)$ and 
%  $V=\sum_\bullet \moule{V}\comoule{B}$ is $\text{simp}_1$, that is:
%  \eq{ X_H = X_c + \sum_\bullet \moule{I}\comoule{B} \longrightarrow
%  \widetilde{X} = X_c + \sum_\bullet \moule{\Sam}\comoule{B},}
% %
% with $\Sam^{\mot{k}}$ defined as before, and  replacing $\omega_j$ by $k^j\cdot\freq$.
% \end{prop}
%%
%\begin{proof}
%We use again the Baker-Campbell-Hausdorff formula; with $\widetilde{X}=\Theta X
%\inv{\Theta}$ we have:
%%
%\eq{\begin{aligned}
%        \widetilde{X} &= X - [X,V] + \dotsm\\
%                            &= X_c + \sum_{k\in\Z^\nu} B_k - [X_c,V] -\dotsm\\
%                            \end{aligned}.}
% Hence we solve $ \sum_{k\in\Z^\nu}B_k = [X_c,V]$ and by setting 
% $V=\sum_{s\geq1}\epsilon^s\sum_{k\in\Z^\nu} \expe{(k\cdot q )}V_k^{(s)}$,
% we find $V_k^{(s)}=\frac{1}{\i(k\cdot\freq)}$.
%%
% \end{proof}
%%
By this way, we are able to perform a trimmed form of a Hamiltonian vector field in action-angle coordinates. It is defined by the mould $\moule{\Tram}$ exactly the same as before.

 Moreover, remark that every simplification is a canonical transformation, so at every
 step of the procedure is the vector field still Hamiltonian. That may be of great interest
 in numerical applications.
 
 
                           
                           

